Hybrid Quantum-Classical Algorithm For Robust Optimization via Stochastic-Gradient Online Learning

Optimization theory has been widely studied in academia and finds a large variety of applications in industry. The different optimization models in their discrete and/or continuous settings have catered to a rich source of research problems. Robust convex optimization is a branch of optimization theory in which the variables or parameters involved have a certain level of uncertainty. In this work, we consider the online robust optimization meta-algorithm by Ben-Tal et al. and show that for a large range of stochastic subgradients, this algorithm has the same guarantee as the original non-stochastic version. We develop a hybrid quantum-classical version of this algorithm and show that an at most quadratic improvement in terms of the dimension can be achieved. The speedup is due to the use of quantum state preparation, quantum norm estimation, and quantum multi-sampling. We apply our quantum meta-algorithm to examples such as robust linear programs and robust semidefinite programs and give applications of these robust optimization problems in finance and engineering.

==> QORO <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{77}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem[\protect\citeauthoryear{Allcock et~al.}{2024}]{allcock2023constant}
\begin{barticle}
\bauthor{\bsnm{Allcock}, \binits{J.}},
\bauthor{\bsnm{Bao}, \binits{J.}},
\bauthor{\bsnm{Doriguello}, \binits{J.F.}},
\bauthor{\bsnm{Luongo}, \binits{A.}},
\bauthor{\bsnm{Santha}, \binits{M.}}:
\batitle{Constant-depth circuits for {B}oolean functions and quantum memory
  devices using multi-qubit gates}.
\bjtitle{{Quantum}}
\bvolume{8},
\bfpage{1530}
(\byear{2024})
\doiurl{10.22331/q-2024-11-20-1530}
\end{barticle}
\endbibitem

%%% 2
\bibitem[\protect\citeauthoryear{Arunachalam
  et~al.}{2015}]{Arunachalam2015robustness}
\begin{barticle}
\bauthor{\bsnm{Arunachalam}, \binits{S.}},
\bauthor{\bsnm{Gheorghiu}, \binits{V.}},
\bauthor{\bsnm{Jochym-O’Connor}, \binits{T.}},
\bauthor{\bsnm{Mosca}, \binits{M.}},
\bauthor{\bsnm{Srinivasan}, \binits{P.V.}}:
\batitle{On the robustness of bucket brigade quantum ram}.
\bjtitle{New Journal of Physics}
\bvolume{17}(\bissue{12}),
\bfpage{123010}
(\byear{2015})
\doiurl{10.1088/1367-2630/17/12/123010}
\end{barticle}
\endbibitem

%%% 3
\bibitem[\protect\citeauthoryear{Arora et~al.}{2012}]{Arora2016}
\begin{bchapter}
\bauthor{\bsnm{Arora}, \binits{S.}},
\bauthor{\bsnm{Ge}, \binits{R.}},
\bauthor{\bsnm{Kannan}, \binits{R.}},
\bauthor{\bsnm{Moitra}, \binits{A.}}:
\bctitle{Computing a nonnegative matrix factorization -- provably}.
In: \bbtitle{Proceedings of the Forty-Fourth Annual ACM Symposium on Theory of
  Computing}.
\bsertitle{STOC '12},
pp. \bfpage{145}--\blpage{162}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{2012}).
\doiurl{10.1145/2213977.2213994}
\end{bchapter}
\endbibitem

%%% 4
\bibitem[\protect\citeauthoryear{{{\DE{Ag}{van}} Apeldoorn} and
  Gily{\'e}n}{2019}]{van2019quantum}
\begin{barticle}
\bauthor{\bsnm{{{\DE{Ag}{van}} Apeldoorn}}, \binits{J.}},
\bauthor{\bsnm{Gily{\'e}n}, \binits{A.}}:
\batitle{Quantum algorithms for zero-sum games}.
\bjtitle{arXiv preprint arXiv:1904.03180}
(\byear{2019})
\doiurl{10.48550/arXiv.1904.03180}
\end{barticle}
\endbibitem

%%% 5
\bibitem[\protect\citeauthoryear{{{\DE{Ag}{van}} Apeldoorn}
  et~al.}{2020}]{VanApeldoorn2020}
\begin{barticle}
\bauthor{\bsnm{{{\DE{Ag}{van}} Apeldoorn}}, \binits{J.}},
\bauthor{\bsnm{Gily{\'{e}}n}, \binits{A.}},
\bauthor{\bsnm{Gribling}, \binits{S.}},
\bauthor{\bsnm{{de Wolf}}, \binits{R.}}:
\batitle{{Quantum SDP-Solvers: Better upper and lower bounds}}.
\bjtitle{Quantum}
\bvolume{4},
\bfpage{1}--\blpage{69}
(\byear{2020})
\doiurl{10.22331/q-2020-02-14-230}
\end{barticle}
\endbibitem

%%% 6
\bibitem[\protect\citeauthoryear{Arora et~al.}{2012}]{arora2012multiplicative}
\begin{barticle}
\bauthor{\bsnm{Arora}, \binits{S.}},
\bauthor{\bsnm{Hazan}, \binits{E.}},
\bauthor{\bsnm{Kale}, \binits{S.}}:
\batitle{The multiplicative weights update method: a meta-algorithm and
  applications}.
\bjtitle{Theory of Computing}
\bvolume{8}(\bissue{6}),
\bfpage{121}--\blpage{164}
(\byear{2012})
\doiurl{10.4086/toc.2012.v008a006}
\end{barticle}
\endbibitem

%%% 7
\bibitem[\protect\citeauthoryear{Arora and Kale}{2007}]{Arora2016a}
\begin{bchapter}
\bauthor{\bsnm{Arora}, \binits{S.}},
\bauthor{\bsnm{Kale}, \binits{S.}}:
\bctitle{A combinatorial, primal-dual approach to semidefinite programs}.
In: \bbtitle{Proceedings of the Thirty-Ninth Annual ACM Symposium on Theory of
  Computing}.
\bsertitle{STOC '07},
pp. \bfpage{227}--\blpage{236}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{2007}).
\doiurl{10.1145/1250790.1250823}
\end{bchapter}
\endbibitem

%%% 8
\bibitem[\protect\citeauthoryear{Arunachalam and
  Maity}{2020}]{arunachalam2020quantum}
\begin{bchapter}
\bauthor{\bsnm{Arunachalam}, \binits{S.}},
\bauthor{\bsnm{Maity}, \binits{R.}}:
\bctitle{Quantum boosting}.
In: \beditor{\bsnm{III}, \binits{H.D.}},
\beditor{\bsnm{Singh}, \binits{A.}} (eds.)
\bbtitle{Proceedings of the 37th International Conference on Machine Learning}.
\bsertitle{Proceedings of Machine Learning Research},
vol. \bseriesno{119},
pp. \bfpage{377}--\blpage{387}.
\bpublisher{PMLR},
\blocation{Vienna, Austria}
(\byear{2020})
\end{bchapter}
\endbibitem

%%% 9
\bibitem[\protect\citeauthoryear{Avant and
  Morgansen}{2023}]{avant2023analytical}
\begin{barticle}
\bauthor{\bsnm{Avant}, \binits{T.}},
\bauthor{\bsnm{Morgansen}, \binits{K.A.}}:
\batitle{Analytical bounds on the local lipschitz constants of relu networks}.
\bjtitle{IEEE Transactions on Neural Networks and Learning Systems}
\bvolume{35}(\bissue{10}),
\bfpage{13902}--\blpage{13913}
(\byear{2023})
\end{barticle}
\endbibitem

%%% 10
\bibitem[\protect\citeauthoryear{Arora}{2009}]{arora2009learning}
\begin{bchapter}
\bauthor{\bsnm{Arora}, \binits{R.}}:
\bctitle{On learning rotations}.
In: \beditor{\bsnm{Bengio}, \binits{Y.}},
\beditor{\bsnm{Schuurmans}, \binits{D.}},
\beditor{\bsnm{Lafferty}, \binits{J.}},
\beditor{\bsnm{Williams}, \binits{C.}},
\beditor{\bsnm{Culotta}, \binits{A.}} (eds.)
\bbtitle{Advances in Neural Information Processing Systems},
vol. \bseriesno{22}.
\bpublisher{Curran Associates, Inc.},
\blocation{Vancouver, BC, Canada}
(\byear{2009})
\end{bchapter}
\endbibitem

%%% 11
\bibitem[\protect\citeauthoryear{Berry et~al.}{2007}]{berry2007efficient}
\begin{barticle}
\bauthor{\bsnm{Berry}, \binits{D.W.}},
\bauthor{\bsnm{Ahokas}, \binits{G.}},
\bauthor{\bsnm{Cleve}, \binits{R.}},
\bauthor{\bsnm{Sanders}, \binits{B.C.}}:
\batitle{Efficient quantum algorithms for simulating sparse {H}amiltonians}.
\bjtitle{Communications in Mathematical Physics}
\bvolume{270}(\bissue{2}),
\bfpage{359}--\blpage{371}
(\byear{2007})
\doiurl{10.1007/s00220-006-0150-x}
\end{barticle}
\endbibitem

%%% 12
\bibitem[\protect\citeauthoryear{Bertsimas et~al.}{2011}]{bertsimas2011theory}
\begin{barticle}
\bauthor{\bsnm{Bertsimas}, \binits{D.}},
\bauthor{\bsnm{Brown}, \binits{D.B.}},
\bauthor{\bsnm{Caramanis}, \binits{C.}}:
\batitle{Theory and applications of robust optimization}.
\bjtitle{SIAM Review}
\bvolume{53}(\bissue{3}),
\bfpage{464}--\blpage{501}
(\byear{2011})
\doiurl{10.1137/080734510}
\end{barticle}
\endbibitem

%%% 13
\bibitem[\protect\citeauthoryear{Berry et~al.}{2014}]{berry2014exponential}
\begin{bchapter}
\bauthor{\bsnm{Berry}, \binits{D.W.}},
\bauthor{\bsnm{Childs}, \binits{A.M.}},
\bauthor{\bsnm{Cleve}, \binits{R.}},
\bauthor{\bsnm{Kothari}, \binits{R.}},
\bauthor{\bsnm{Somma}, \binits{R.D.}}:
\bctitle{Exponential improvement in precision for simulating sparse
  {H}amiltonians}.
In: \bbtitle{Proceedings of the Forty-Sixth Annual ACM Symposium on Theory of
  Computing}.
\bsertitle{STOC '14},
pp. \bfpage{283}--\blpage{292}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{2014}).
\doiurl{10.1145/2591796.2591854}
\end{bchapter}
\endbibitem

%%% 14
\bibitem[\protect\citeauthoryear{Brassard et~al.}{2011}]{brassard2011optimal}
\begin{barticle}
\bauthor{\bsnm{Brassard}, \binits{G.}},
\bauthor{\bsnm{Dupuis}, \binits{F.}},
\bauthor{\bsnm{Gambs}, \binits{S.}},
\bauthor{\bsnm{Tapp}, \binits{A.}}:
\batitle{An optimal quantum algorithm to approximate the mean and its
  application for approximating the median of a set of points over an arbitrary
  distance}.
\bjtitle{arXiv preprint arXiv:1106.4267}
(\byear{2011})
\doiurl{10.48550/arXiv.1106.4267}
\end{barticle}
\endbibitem

%%% 15
\bibitem[\protect\citeauthoryear{Bhowmick et~al.}{2021}]{bhowmick2021lipbab}
\begin{bchapter}
\bauthor{\bsnm{Bhowmick}, \binits{A.}},
\bauthor{\bsnm{D’Souza}, \binits{M.}},
\bauthor{\bsnm{Raghavan}, \binits{G.S.}}:
\bctitle{Lipbab: Computing exact lipschitz constant of relu networks}.
In: \bbtitle{International Conference on Artificial Neural Networks},
pp. \bfpage{151}--\blpage{162}
(\byear{2021}).
\bcomment{Springer}
\end{bchapter}
\endbibitem

%%% 16
\bibitem[\protect\citeauthoryear{Babbush et~al.}{2018}]{babbush2018encoding}
\begin{barticle}
\bauthor{\bsnm{Babbush}, \binits{R.}},
\bauthor{\bsnm{Gidney}, \binits{C.}},
\bauthor{\bsnm{Berry}, \binits{D.W.}},
\bauthor{\bsnm{Wiebe}, \binits{N.}},
\bauthor{\bsnm{McClean}, \binits{J.}},
\bauthor{\bsnm{Paler}, \binits{A.}},
\bauthor{\bsnm{Fowler}, \binits{A.}},
\bauthor{\bsnm{Neven}, \binits{H.}}:
\batitle{Encoding electronic spectra in quantum circuits with linear t
  complexity}.
\bjtitle{Phys. Rev. X}
\bvolume{8},
\bfpage{041015}
(\byear{2018})
\doiurl{10.1103/PhysRevX.8.041015}
\end{barticle}
\endbibitem

%%% 17
\bibitem[\protect\citeauthoryear{Brassard et~al.}{2002}]{Brassard2002}
\begin{barticle}
\bauthor{\bsnm{Brassard}, \binits{G.}},
\bauthor{\bsnm{H{\o}yer}, \binits{P.}},
\bauthor{\bsnm{Mosca}, \binits{M.}},
\bauthor{\bsnm{Tapp}, \binits{A.}}:
\batitle{Quantum amplitude amplification and estimation}.
\bjtitle{Contemporary Mathematics}
\bvolume{305},
\bfpage{53}--\blpage{74}
(\byear{2002})
\doiurl{10.1090/conm/305/05215}
\end{barticle}
\endbibitem

%%% 18
\bibitem[\protect\citeauthoryear{Belmega et~al.}{2022}]{belmega2022online}
\begin{bchapter}
\bauthor{\bsnm{Belmega}, \binits{E.V.}},
\bauthor{\bsnm{Mertikopoulos}, \binits{P.}},
\bauthor{\bsnm{Negrel}, \binits{R.}}:
\bctitle{Online convex optimization in wireless networks and beyond: The
  feedback-performance trade-off}.
In: \bbtitle{2022 20th International Symposium on Modeling and Optimization in
  Mobile, Ad Hoc, and Wireless Networks (WiOpt)},
pp. \bfpage{298}--\blpage{305}
(\byear{2022}).
\doiurl{10.23919/WiOpt56218.2022.9930534}
\end{bchapter}
\endbibitem

%%% 19
\bibitem[\protect\citeauthoryear{Bottou}{1999}]{bottou1998online}
\begin{bbook}
\bauthor{\bsnm{Bottou}, \binits{L.}}:
\bbtitle{On-line learning and stochastic approximations},
pp. \bfpage{9}--\blpage{42}.
\bpublisher{Cambridge University Press},
\blocation{USA}
(\byear{1999})
\end{bbook}
\endbibitem

%%% 20
\bibitem[\protect\citeauthoryear{Brandao and Svore}{2017}]{Brandao2017}
\begin{bchapter}
\bauthor{\bsnm{Brandao}, \binits{F.G.S.L.}},
\bauthor{\bsnm{Svore}, \binits{K.M.}}:
\bctitle{Quantum speed-ups for solving semidefinite programs}.
In: \bbtitle{2017 IEEE 58th Annual Symposium on Foundations of Computer Science
  (FOCS)},
pp. \bfpage{415}--\blpage{426}
(\byear{2017}).
\doiurl{10.1109/FOCS.2017.45}
\end{bchapter}
\endbibitem

%%% 21
\bibitem[\protect\citeauthoryear{Bertsimas and
  Thiele}{2004}]{bertsimas2004robust}
\begin{bchapter}
\bauthor{\bsnm{Bertsimas}, \binits{D.}},
\bauthor{\bsnm{Thiele}, \binits{A.}}:
\bctitle{A robust optimization approach to supply chain management}.
In: \beditor{\bsnm{Bienstock}, \binits{D.}},
\beditor{\bsnm{Nemhauser}, \binits{G.}} (eds.)
\bbtitle{Integer Programming and Combinatorial Optimization},
pp. \bfpage{86}--\blpage{100}.
\bpublisher{Springer},
\blocation{Berlin, Heidelberg}
(\byear{2004})
\end{bchapter}
\endbibitem

%%% 22
\bibitem[\protect\citeauthoryear{Ben-Tal et~al.}{2000}]{ben2000robust}
\begin{bchapter}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{El~Ghaoui}, \binits{L.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\bctitle{Robustness}.
In: \beditor{\bsnm{Wolkowicz}, \binits{H.}},
\beditor{\bsnm{Saigal}, \binits{R.}},
\beditor{\bsnm{Vandenberghe}, \binits{L.}} (eds.)
\bbtitle{Handbook of Semidefinite Programming: Theory, Algorithms, and
  Applications},
pp. \bfpage{139}--\blpage{162}.
\bpublisher{Springer},
\blocation{Boston, MA}
(\byear{2000}).
\doiurl{10.1007/978-1-4615-4381-7_6}
\end{bchapter}
\endbibitem

%%% 23
\bibitem[\protect\citeauthoryear{Ben-Tal et~al.}{2009}]{ben2009robust}
\begin{bbook}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Ghaoui}, \binits{L.E.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\bbtitle{Robust Optimization}.
\bpublisher{Princeton University Press},
\blocation{Princeton}
(\byear{2009}).
\doiurl{10.1515/9781400831050}
\end{bbook}
\endbibitem

%%% 24
\bibitem[\protect\citeauthoryear{Ben-Tal et~al.}{2015}]{Ben-Tal2015a}
\begin{barticle}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Hazan}, \binits{E.}},
\bauthor{\bsnm{Koren}, \binits{T.}},
\bauthor{\bsnm{Mannor}, \binits{S.}}:
\batitle{{Oracle-based robust optimization via online learning}}.
\bjtitle{Operations Research}
\bvolume{63}(\bissue{3}),
\bfpage{628}--\blpage{638}
(\byear{2015})
\doiurl{10.1287/opre.2015.1374}
\end{barticle}
\endbibitem

%%% 25
\bibitem[\protect\citeauthoryear{Ben-Tal and Nemirovski}{1997}]{ben1997robust}
\begin{barticle}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\batitle{Robust truss topology design via semidefinite programming}.
\bjtitle{SIAM Journal on Optimization}
\bvolume{7}(\bissue{4}),
\bfpage{991}--\blpage{1016}
(\byear{1997})
\doiurl{10.1137/S1052623495291951}
\end{barticle}
\endbibitem

%%% 26
\bibitem[\protect\citeauthoryear{Ben-Tal and Nemirovski}{1998}]{ben1998robust}
\begin{barticle}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\batitle{Robust convex optimization}.
\bjtitle{Mathematics of Operations Research}
\bvolume{23}(\bissue{4}),
\bfpage{769}--\blpage{805}
(\byear{1998})
\doiurl{10.1287/moor.23.4.769}
\end{barticle}
\endbibitem

%%% 27
\bibitem[\protect\citeauthoryear{Ben-Tal and Nemirovski}{1999}]{ben1999robust}
\begin{barticle}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\batitle{Robust solutions of uncertain linear programs}.
\bjtitle{Operations Research Letters}
\bvolume{25}(\bissue{1}),
\bfpage{1}--\blpage{13}
(\byear{1999})
\doiurl{10.1016/S0167-6377(99)00016-4}
\end{barticle}
\endbibitem

%%% 28
\bibitem[\protect\citeauthoryear{Ben-Tal and
  Nemirovski}{2001}]{ben2001lectures}
\begin{bbook}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\bbtitle{Lectures on Modern Convex Optimization}.
\bpublisher{Society for Industrial and Applied Mathematics},
\blocation{USA}
(\byear{2001}).
\doiurl{10.1137/1.9780898718829}
\end{bbook}
\endbibitem

%%% 29
\bibitem[\protect\citeauthoryear{Ben-Tal and Nemirovski}{2002}]{ben2002robust}
\begin{barticle}
\bauthor{\bsnm{Ben-Tal}, \binits{A.}},
\bauthor{\bsnm{Nemirovski}, \binits{A.}}:
\batitle{Robust optimization -- methodology and applications}.
\bjtitle{Mathematical Programming}
\bvolume{92}(\bissue{3}),
\bfpage{453}--\blpage{480}
(\byear{2002})
\doiurl{10.1007/s101070100286}
\end{barticle}
\endbibitem

%%% 30
\bibitem[\protect\citeauthoryear{Bellante et~al.}{2025}]{bellante2025quantum}
\begin{botherref}
\oauthor{\bsnm{Bellante}, \binits{A.}},
\oauthor{\bsnm{Vanerio}, \binits{S.}},
\oauthor{\bsnm{Zanero}, \binits{S.}}:
Quantum sparse recovery and quantum orthogonal matching pursuit.
arXiv preprint arXiv:2510.06925
(2025)
\end{botherref}
\endbibitem

%%% 31
\bibitem[\protect\citeauthoryear{Cesa-Bianchi and
  Lugosi}{2006}]{cesa2006prediction}
\begin{bbook}
\bauthor{\bsnm{Cesa-Bianchi}, \binits{N.}},
\bauthor{\bsnm{Lugosi}, \binits{G.}}:
\bbtitle{Prediction, Learning, and Games}.
\bpublisher{Cambridge University Press},
\blocation{USA}
(\byear{2006})
\end{bbook}
\endbibitem

%%% 32
\bibitem[\protect\citeauthoryear{Clarkson et~al.}{2012}]{clarkson2012sublinear}
\begin{barticle}
\bauthor{\bsnm{Clarkson}, \binits{K.L.}},
\bauthor{\bsnm{Hazan}, \binits{E.}},
\bauthor{\bsnm{Woodruff}, \binits{D.P.}}:
\batitle{Sublinear optimization for machine learning}.
\bjtitle{Journal of the ACM (JACM)}
\bvolume{59}(\bissue{5}),
\bfpage{1}--\blpage{49}
(\byear{2012})
\doiurl{10.1145/2371656.2371658}
\end{barticle}
\endbibitem

%%% 33
\bibitem[\protect\citeauthoryear{Chen et~al.}{2020}]{chen2020semialgebraic}
\begin{barticle}
\bauthor{\bsnm{Chen}, \binits{T.}},
\bauthor{\bsnm{Lasserre}, \binits{J.B.}},
\bauthor{\bsnm{Magron}, \binits{V.}},
\bauthor{\bsnm{Pauwels}, \binits{E.}}:
\batitle{Semialgebraic optimization for lipschitz constants of relu networks}.
\bjtitle{Advances in Neural Information Processing Systems}
\bvolume{33},
\bfpage{19189}--\blpage{19200}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 34
\bibitem[\protect\citeauthoryear{Chen et~al.}{2024}]{chen2024low}
\begin{botherref}
\oauthor{\bsnm{Chen}, \binits{Z.}},
\oauthor{\bsnm{Sheehan}, \binits{C.}},
\oauthor{\bsnm{Zadik}, \binits{I.}}:
On the low-temperature mcmc threshold: the cases of sparse tensor {PCA}, sparse
  regression, and a geometric rule.
arXiv preprint arXiv:2408.00746
(2024)
\end{botherref}
\endbibitem

%%% 35
\bibitem[\protect\citeauthoryear{Chopra and Ziemba}{1993}]{chopra2013effect}
\begin{barticle}
\bauthor{\bsnm{Chopra}, \binits{V.K.}},
\bauthor{\bsnm{Ziemba}, \binits{W.T.}}:
\batitle{The effect of errors in means, variances, and covariances on optimal
  portfolio choice}.
\bjtitle{The Journal of Portfolio Management}
\bvolume{19},
\bfpage{6}--\blpage{11}
(\byear{1993})
\doiurl{10.3905/jpm.1993.409440}
\end{barticle}
\endbibitem

%%% 36
\bibitem[\protect\citeauthoryear{Doriguello
  et~al.}{2025}]{Doriguello2025quantumalgorithms}
\begin{barticle}
\bauthor{\bsnm{Doriguello}, \binits{J.F.}},
\bauthor{\bsnm{Lim}, \binits{D.}},
\bauthor{\bsnm{Pun}, \binits{C.S.}},
\bauthor{\bsnm{Rebentrost}, \binits{P.}},
\bauthor{\bsnm{Vaidya}, \binits{T.}}:
\batitle{Quantum {A}lgorithms for the {P}athwise {L}asso}.
\bjtitle{{Quantum}}
\bvolume{9},
\bfpage{1674}
(\byear{2025})
\doiurl{10.22331/q-2025-03-25-1674}
\end{barticle}
\endbibitem

%%% 37
\bibitem[\protect\citeauthoryear{Duchi et~al.}{2008}]{duchi2008efficient}
\begin{bchapter}
\bauthor{\bsnm{Duchi}, \binits{J.}},
\bauthor{\bsnm{Shalev-Shwartz}, \binits{S.}},
\bauthor{\bsnm{Singer}, \binits{Y.}},
\bauthor{\bsnm{Chandra}, \binits{T.}}:
\bctitle{Efficient projections onto the $l_1$-ball for learning in high
  dimensions}.
In: \bbtitle{Proceedings of the 25th International Conference on Machine
  Learning}.
\bsertitle{ICML '08},
pp. \bfpage{272}--\blpage{279}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{2008}).
\doiurl{10.1145/1390156.1390191}
\end{bchapter}
\endbibitem

%%% 38
\bibitem[\protect\citeauthoryear{Flaxman et~al.}{2005}]{Flaxman2004}
\begin{bchapter}
\bauthor{\bsnm{Flaxman}, \binits{A.D.}},
\bauthor{\bsnm{Kalai}, \binits{A.T.}},
\bauthor{\bsnm{McMahan}, \binits{H.B.}}:
\bctitle{Online convex optimization in the bandit setting: gradient descent
  without a gradient}.
In: \bbtitle{Proceedings of the Sixteenth Annual ACM-SIAM Symposium on Discrete
  Algorithms}.
\bsertitle{SODA '05},
pp. \bfpage{385}--\blpage{394}.
\bpublisher{Society for Industrial and Applied Mathematics},
\blocation{USA}
(\byear{2005})
\end{bchapter}
\endbibitem

%%% 39
\bibitem[\protect\citeauthoryear{Fotakis et~al.}{2020}]{Fotakis2020}
\begin{bchapter}
\bauthor{\bsnm{Fotakis}, \binits{D.}},
\bauthor{\bsnm{Lianeas}, \binits{T.}},
\bauthor{\bsnm{Piliouras}, \binits{G.}},
\bauthor{\bsnm{Skoulakis}, \binits{S.}}:
\bctitle{Efficient online learning of optimal rankings: Dimensionality
  reduction via gradient descent}.
In: \beditor{\bsnm{Larochelle}, \binits{H.}},
\beditor{\bsnm{Ranzato}, \binits{M.}},
\beditor{\bsnm{Hadsell}, \binits{R.}},
\beditor{\bsnm{Balcan}, \binits{M.F.}},
\beditor{\bsnm{Lin}, \binits{H.}} (eds.)
\bbtitle{Advances in Neural Information Processing Systems},
vol. \bseriesno{33},
pp. \bfpage{7816}--\blpage{7827}.
\bpublisher{Curran Associates, Inc.},
\blocation{Virtual}
(\byear{2020})
\end{bchapter}
\endbibitem

%%% 40
\bibitem[\protect\citeauthoryear{Freund and Schapire}{1997}]{Freund1997}
\begin{barticle}
\bauthor{\bsnm{Freund}, \binits{Y.}},
\bauthor{\bsnm{Schapire}, \binits{R.E.}}:
\batitle{A decision-theoretic generalization of on-line learning and an
  application to boosting}.
\bjtitle{Journal of Computer and System Sciences}
\bvolume{55}(\bissue{1}),
\bfpage{119}--\blpage{139}
(\byear{1997})
\doiurl{10.1006/jcss.1997.1504}
\end{barticle}
\endbibitem

%%% 41
\bibitem[\protect\citeauthoryear{Geoffrey et~al.}{2020}]{geoffrey2020robust}
\begin{barticle}
\bauthor{\bsnm{Geoffrey}, \binits{C.}},
\bauthor{\bsnm{Guillaume}, \binits{L.}},
\bauthor{\bsnm{Matthieu}, \binits{L.}}:
\batitle{Robust high dimensional learning for lipschitz and convex losses}.
\bjtitle{Journal of Machine Learning Research}
\bvolume{21}(\bissue{233}),
\bfpage{1}--\blpage{47}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 42
\bibitem[\protect\citeauthoryear{Goldfarb and
  Iyengar}{2003}]{goldfarb2003robust}
\begin{barticle}
\bauthor{\bsnm{Goldfarb}, \binits{D.}},
\bauthor{\bsnm{Iyengar}, \binits{G.}}:
\batitle{Robust portfolio selection problems}.
\bjtitle{Mathematics of Operations Research}
\bvolume{28}(\bissue{1}),
\bfpage{1}--\blpage{38}
(\byear{2003})
\doiurl{10.1287/moor.28.1.1.14260}
\end{barticle}
\endbibitem

%%% 43
\bibitem[\protect\citeauthoryear{Grigoriadis and
  Khachiyan}{1995}]{Grigoriadis1995}
\begin{barticle}
\bauthor{\bsnm{Grigoriadis}, \binits{M.D.}},
\bauthor{\bsnm{Khachiyan}, \binits{L.G.}}:
\batitle{{A sublinear-time randomized approximation algorithm for matrix
  games}}.
\bjtitle{Operations Research Letters}
\bvolume{18}(\bissue{2}),
\bfpage{53}--\blpage{58}
(\byear{1995})
\doiurl{10.1016/0167-6377(95)00032-0}
\end{barticle}
\endbibitem

%%% 44
\bibitem[\protect\citeauthoryear{Giovannetti
  et~al.}{2008a}]{giovannetti2008architectures}
\begin{barticle}
\bauthor{\bsnm{Giovannetti}, \binits{V.}},
\bauthor{\bsnm{Lloyd}, \binits{S.}},
\bauthor{\bsnm{Maccone}, \binits{L.}}:
\batitle{Architectures for a quantum random access memory}.
\bjtitle{Phys. Rev. A}
\bvolume{78},
\bfpage{052310}
(\byear{2008})
\doiurl{10.1103/PhysRevA.78.052310}
\end{barticle}
\endbibitem

%%% 45
\bibitem[\protect\citeauthoryear{Giovannetti
  et~al.}{2008b}]{giovannetti2008quantum}
\begin{barticle}
\bauthor{\bsnm{Giovannetti}, \binits{V.}},
\bauthor{\bsnm{Lloyd}, \binits{S.}},
\bauthor{\bsnm{Maccone}, \binits{L.}}:
\batitle{Quantum random access memory}.
\bjtitle{Phys. Rev. Lett.}
\bvolume{100},
\bfpage{160501}
(\byear{2008})
\doiurl{10.1103/PhysRevLett.100.160501}
\end{barticle}
\endbibitem

%%% 46
\bibitem[\protect\citeauthoryear{Gily\'{e}n et~al.}{2019}]{gilyen2019quantum}
\begin{bchapter}
\bauthor{\bsnm{Gily\'{e}n}, \binits{A.}},
\bauthor{\bsnm{Su}, \binits{Y.}},
\bauthor{\bsnm{Low}, \binits{G.H.}},
\bauthor{\bsnm{Wiebe}, \binits{N.}}:
\bctitle{Quantum singular value transformation and beyond: exponential
  improvements for quantum matrix arithmetics}.
In: \bbtitle{Proceedings of the 51st Annual ACM SIGACT Symposium on Theory of
  Computing}.
\bsertitle{STOC 2019},
pp. \bfpage{193}--\blpage{204}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{2019}).
\doiurl{10.1145/3313276.3316366}
\end{bchapter}
\endbibitem

%%% 47
\bibitem[\protect\citeauthoryear{Hazan et~al.}{2007}]{hazan2007logarithmic}
\begin{barticle}
\bauthor{\bsnm{Hazan}, \binits{E.}},
\bauthor{\bsnm{Agarwal}, \binits{A.}},
\bauthor{\bsnm{Kale}, \binits{S.}}:
\batitle{Logarithmic regret algorithms for online convex optimization}.
\bjtitle{Machine Learning}
\bvolume{69}(\bissue{2}),
\bfpage{169}--\blpage{192}
(\byear{2007})
\doiurl{10.1007/s10994-007-5016-8}
\end{barticle}
\endbibitem

%%% 48
\bibitem[\protect\citeauthoryear{Hamoudi}{2022}]{hamoudi2022preparing}
\begin{barticle}
\bauthor{\bsnm{Hamoudi}, \binits{Y.}}:
\batitle{Preparing many copies of a quantum state in the black-box model}.
\bjtitle{Phys. Rev. A}
\bvolume{105},
\bfpage{062440}
(\byear{2022})
\doiurl{10.1103/PhysRevA.105.062440}
\end{barticle}
\endbibitem

%%% 49
\bibitem[\protect\citeauthoryear{Hazan}{2016}]{Hazan2016b}
\begin{barticle}
\bauthor{\bsnm{Hazan}, \binits{E.}}:
\batitle{{Introduction to Online Convex Optimization}}.
\bjtitle{Foundations and Trends{\textregistered} in Optimization}
\bvolume{2}(\bissue{3-4}),
\bfpage{157}--\blpage{325}
(\byear{2016})
\doiurl{10.1561/2400000013}
\end{barticle}
\endbibitem

%%% 50
\bibitem[\protect\citeauthoryear{Harrow et~al.}{2009}]{harrow2009quantum}
\begin{barticle}
\bauthor{\bsnm{Harrow}, \binits{A.W.}},
\bauthor{\bsnm{Hassidim}, \binits{A.}},
\bauthor{\bsnm{Lloyd}, \binits{S.}}:
\batitle{Quantum algorithm for linear systems of equations}.
\bjtitle{Phys. Rev. Lett.}
\bvolume{103},
\bfpage{150502}
(\byear{2009})
\doiurl{10.1103/PhysRevLett.103.150502}
\end{barticle}
\endbibitem

%%% 51
\bibitem[\protect\citeauthoryear{Hazan et~al.}{2016}]{Hazan2016a}
\begin{barticle}
\bauthor{\bsnm{Hazan}, \binits{E.}},
\bauthor{\bsnm{Kale}, \binits{S.}},
\bauthor{\bsnm{Warmuth}, \binits{M.K.}}:
\batitle{{Learning rotations with little regret}}.
\bjtitle{Machine Learning}
\bvolume{104}(\bissue{1}),
\bfpage{129}--\blpage{148}
(\byear{2016})
\doiurl{10.1007/s10994-016-5548-x}
\end{barticle}
\endbibitem

%%% 52
\bibitem[\protect\citeauthoryear{Hamoudi et~al.}{2019}]{Hamoudi2019}
\begin{barticle}
\bauthor{\bsnm{Hamoudi}, \binits{Y.}},
\bauthor{\bsnm{Rebentrost}, \binits{P.}},
\bauthor{\bsnm{Rosmanis}, \binits{A.}},
\bauthor{\bsnm{Santha}, \binits{M.}}:
\batitle{{Quantum and classical algorithms for approximate submodular function
  minimization}}.
\bjtitle{Quantum Information and Computation}
\bvolume{19}(\bissue{15-16}),
\bfpage{1325}--\blpage{1349}
(\byear{2019})
\doiurl{10.26421/qic19.15-16-5}
\end{barticle}
\endbibitem

%%% 53
\bibitem[\protect\citeauthoryear{Helmbold et~al.}{1998}]{Helmbold1998}
\begin{barticle}
\bauthor{\bsnm{Helmbold}, \binits{D.P.}},
\bauthor{\bsnm{Schapire}, \binits{R.E.}},
\bauthor{\bsnm{Singer}, \binits{Y.}},
\bauthor{\bsnm{Warmuth}, \binits{M.K.}}:
\batitle{{On-line portfolio selection using multiplicative updates}}.
\bjtitle{Mathematical Finance}
\bvolume{8}(\bissue{4}),
\bfpage{325}--\blpage{347}
(\byear{1998})
\doiurl{10.1111/1467-9965.00058}
\end{barticle}
\endbibitem

%%% 54
\bibitem[\protect\citeauthoryear{Helmbold and Warmuth}{2007}]{Hazan2007}
\begin{bchapter}
\bauthor{\bsnm{Helmbold}, \binits{D.P.}},
\bauthor{\bsnm{Warmuth}, \binits{M.K.}}:
\bctitle{Learning permutations with exponential weights}.
In: \beditor{\bsnm{Bshouty}, \binits{N.H.}},
\beditor{\bsnm{Gentile}, \binits{C.}} (eds.)
\bbtitle{Learning Theory},
pp. \bfpage{469}--\blpage{483}.
\bpublisher{Springer},
\blocation{Berlin, Heidelberg}
(\byear{2007}).
\doiurl{10.1007/978-3-540-72927-3_34}
\end{bchapter}
\endbibitem

%%% 55
\bibitem[\protect\citeauthoryear{Helmbold and Warmuth}{2009}]{Helmbold2009}
\begin{barticle}
\bauthor{\bsnm{Helmbold}, \binits{D.P.}},
\bauthor{\bsnm{Warmuth}, \binits{M.K.}}:
\batitle{Learning permutations with exponential weights}.
\bjtitle{J. Mach. Learn. Res.}
\bvolume{10},
\bfpage{1705}--\blpage{1736}
(\byear{2009})
\end{barticle}
\endbibitem

%%% 56
\bibitem[\protect\citeauthoryear{Izdebski and {de
  Wolf}}{2023}]{izdebski2020improved}
\begin{bchapter}
\bauthor{\bsnm{Izdebski}, \binits{A.}},
\bauthor{\bsnm{{de Wolf}}, \binits{R.}}:
\bctitle{{Improved Quantum Boosting}}.
In: \beditor{\bsnm{G{\o}rtz}, \binits{I.L.}},
\beditor{\bsnm{Farach-Colton}, \binits{M.}},
\beditor{\bsnm{Puglisi}, \binits{S.J.}},
\beditor{\bsnm{Herman}, \binits{G.}} (eds.)
\bbtitle{31st Annual European Symposium on Algorithms (ESA 2023)}.
\bsertitle{Leibniz International Proceedings in Informatics (LIPIcs)},
vol. \bseriesno{274},
pp. \bfpage{64}--\blpage{16416}.
\bpublisher{Schloss Dagstuhl -- Leibniz-Zentrum f{\"u}r Informatik},
\blocation{Dagstuhl, Germany}
(\byear{2023}).
\doiurl{10.4230/LIPIcs.ESA.2023.64}
\end{bchapter}
\endbibitem

%%% 57
\bibitem[\protect\citeauthoryear{Kim and Giannakis}{2017}]{kim2016online}
\begin{barticle}
\bauthor{\bsnm{Kim}, \binits{S.-J.}},
\bauthor{\bsnm{Giannakis}, \binits{G.B.}}:
\batitle{An online convex optimization approach to real-time energy pricing for
  demand response}.
\bjtitle{IEEE Transactions on Smart Grid}
\bvolume{8}(\bissue{6}),
\bfpage{2784}--\blpage{2793}
(\byear{2017})
\doiurl{10.1109/TSG.2016.2539948}
\end{barticle}
\endbibitem

%%% 58
\bibitem[\protect\citeauthoryear{Korn and M{\"u}ller}{2022}]{Korn2022}
\begin{barticle}
\bauthor{\bsnm{Korn}, \binits{R.}},
\bauthor{\bsnm{M{\"u}ller}, \binits{L.}}:
\batitle{Optimal portfolios in the presence of stress scenarios a worst-case
  approach}.
\bjtitle{Mathematics and Financial Economics}
\bvolume{16}(\bissue{1}),
\bfpage{153}--\blpage{185}
(\byear{2022})
\doiurl{10.1007/s11579-021-00304-2}
\end{barticle}
\endbibitem

%%% 59
\bibitem[\protect\citeauthoryear{Lobo and Boyd}{2000}]{lobo2000worst}
\begin{botherref}
\oauthor{\bsnm{Lobo}, \binits{M.S.}},
\oauthor{\bsnm{Boyd}, \binits{S.}}:
The worst-case risk of a portfolio
(2000)
\end{botherref}
\endbibitem

%%% 60
\bibitem[\protect\citeauthoryear{Li et~al.}{2019}]{li2019sublinear}
\begin{bchapter}
\bauthor{\bsnm{Li}, \binits{T.}},
\bauthor{\bsnm{Chakrabarti}, \binits{S.}},
\bauthor{\bsnm{Wu}, \binits{X.}}:
\bctitle{Sublinear quantum algorithms for training linear and kernel-based
  classifiers}.
In: \beditor{\bsnm{Chaudhuri}, \binits{K.}},
\beditor{\bsnm{Salakhutdinov}, \binits{R.}} (eds.)
\bbtitle{Proceedings of the 36th International Conference on Machine Learning}.
\bsertitle{Proceedings of Machine Learning Research},
vol. \bseriesno{97},
pp. \bfpage{3815}--\blpage{3824}.
\bpublisher{PMLR},
\blocation{Long Beach, California, USA}
(\byear{2019}).
\burl{https://proceedings.mlr.press/v97/li19b.html}
\end{bchapter}
\endbibitem

%%% 61
\bibitem[\protect\citeauthoryear{Li and Hoi}{2014}]{li2014online}
\begin{botherref}
\oauthor{\bsnm{Li}, \binits{B.}},
\oauthor{\bsnm{Hoi}, \binits{S.C.H.}}:
Online portfolio selection: A survey.
ACM Comput. Surv.
\textbf{46}(3)
(2014)
\doiurl{10.1145/2512962}
\end{botherref}
\endbibitem

%%% 62
\bibitem[\protect\citeauthoryear{Luo et~al.}{2025}]{luo2025space}
\begin{botherref}
\oauthor{\bsnm{Luo}, \binits{J.}},
\oauthor{\bsnm{Li}, \binits{G.}},
\oauthor{\bsnm{Li}, \binits{L.}}:
Space-time tradeoff for sparse quantum state preparation.
arXiv preprint arXiv:2506.16964
(2025)
\end{botherref}
\endbibitem

%%% 63
\bibitem[\protect\citeauthoryear{Liu et~al.}{2017}]{liu2017survey}
\begin{barticle}
\bauthor{\bsnm{Liu}, \binits{X.}},
\bauthor{\bsnm{Lu}, \binits{P.}},
\bauthor{\bsnm{Pan}, \binits{B.}}:
\batitle{Survey of convex optimization for aerospace applications}.
\bjtitle{Astrodynamics}
\bvolume{1},
\bfpage{23}--\blpage{40}
(\byear{2017})
\doiurl{10.1007/s42064-017-0003-8}
\end{barticle}
\endbibitem

%%% 64
\bibitem[\protect\citeauthoryear{Markowitz}{1952}]{HarryMarkowitz1952}
\begin{barticle}
\bauthor{\bsnm{Markowitz}, \binits{H.}}:
\batitle{Portfolio selection}.
\bjtitle{The Journal of Finance}
\bvolume{7}(\bissue{1}),
\bfpage{77}--\blpage{91}
(\byear{1952})
\doiurl{10.2307/2975974}
\end{barticle}
\endbibitem

%%% 65
\bibitem[\protect\citeauthoryear{McMahan and
  Streeter}{2010}]{mcmahan2010adaptive}
\begin{bchapter}
\bauthor{\bsnm{McMahan}, \binits{H.B.}},
\bauthor{\bsnm{Streeter}, \binits{M.J.}}:
\bctitle{Adaptive bound optimization for online convex optimization}.
In: \bbtitle{{COLT} 2010 - The 23rd Conference on Learning Theory},
pp. \bfpage{244}--\blpage{256}.
\bpublisher{Omnipress},
\blocation{Haifa, Israel,}
(\byear{2010})
\end{bchapter}
\endbibitem

%%% 66
\bibitem[\protect\citeauthoryear{Mukhopadhyay}{2025}]{Mukhopadhyay2025quantum}
\begin{barticle}
\bauthor{\bsnm{Mukhopadhyay}, \binits{P.}}:
\batitle{A quantum random access memory ({QRAM}) using a polynomial encoding of
  binary strings}.
\bjtitle{Scientific Reports}
\bvolume{15}(\bissue{1}),
\bfpage{11002}
(\byear{2025})
\doiurl{10.1038/s41598-025-95283-5}
\end{barticle}
\endbibitem

%%% 67
\bibitem[\protect\citeauthoryear{Meng et~al.}{2024}]{meng2024lipschitz}
\begin{botherref}
\oauthor{\bsnm{Meng}, \binits{K.}},
\oauthor{\bsnm{Wu}, \binits{P.}},
\oauthor{\bsnm{Yang}, \binits{X.}}:
Lipschitz continuity of solution multifunctions of extended $\ell_1$
  regularization problems.
arXiv preprint arXiv:2406.16053
(2024)
\end{botherref}
\endbibitem

%%% 68
\bibitem[\protect\citeauthoryear{Nielsen and Chuang}{2010}]{nielsen2010quantum}
\begin{bbook}
\bauthor{\bsnm{Nielsen}, \binits{M.A.}},
\bauthor{\bsnm{Chuang}, \binits{I.L.}}:
\bbtitle{Quantum Computation and Quantum Information}.
\bpublisher{Cambridge university press},
\blocation{New Yok}
(\byear{2010}).
\doiurl{10.1017/CBO9780511976667}
\end{bbook}
\endbibitem

%%% 69
\bibitem[\protect\citeauthoryear{Nayak and Wu}{1999}]{nayak1999quantum}
\begin{bchapter}
\bauthor{\bsnm{Nayak}, \binits{A.}},
\bauthor{\bsnm{Wu}, \binits{F.}}:
\bctitle{The quantum query complexity of approximating the median and related
  statistics}.
In: \bbtitle{Proceedings of the Thirty-First Annual ACM Symposium on Theory of
  Computing}.
\bsertitle{STOC '99},
pp. \bfpage{384}--\blpage{393}.
\bpublisher{Association for Computing Machinery},
\blocation{New York, NY, USA}
(\byear{1999}).
\doiurl{10.1145/301250.301349}
\end{bchapter}
\endbibitem

%%% 70
\bibitem[\protect\citeauthoryear{Patel and Goulart}{2011}]{patel2011trajectory}
\begin{barticle}
\bauthor{\bsnm{Patel}, \binits{R.B.}},
\bauthor{\bsnm{Goulart}, \binits{P.J.}}:
\batitle{Trajectory generation for aircraft avoidance maneuvers using online
  optimization}.
\bjtitle{Journal of guidance, control, and dynamics}
\bvolume{34}(\bissue{1}),
\bfpage{218}--\blpage{230}
(\byear{2011})
\doiurl{10.2514/1.49518}
\end{barticle}
\endbibitem

%%% 71
\bibitem[\protect\citeauthoryear{Prakash}{2014}]{prakash2014quantum}
\begin{botherref}
\oauthor{\bsnm{Prakash}, \binits{A.}}:
Quantum algorithms for linear algebra and machine learning.
PhD thesis,
University of California, Berkeley
(2014).
\url{https://escholarship.org/uc/item/5v9535q4}
\end{botherref}
\endbibitem

%%% 72
\bibitem[\protect\citeauthoryear{Servedio}{2001}]{servedio2003smooth}
\begin{bchapter}
\bauthor{\bsnm{Servedio}, \binits{R.A.}}:
\bctitle{Smooth boosting and learning with malicious noise}.
In: \beditor{\bsnm{Helmbold}, \binits{D.}},
\beditor{\bsnm{Williamson}, \binits{B.}} (eds.)
\bbtitle{Computational Learning Theory},
pp. \bfpage{473}--\blpage{489}.
\bpublisher{Springer},
\blocation{Berlin, Heidelberg}
(\byear{2001}).
\doiurl{10.1007/3-540-44581-1_31}
\end{bchapter}
\endbibitem

%%% 73
\bibitem[\protect\citeauthoryear{Shalev-Shwartz}{2012}]{shalev2012online}
\begin{barticle}
\bauthor{\bsnm{Shalev-Shwartz}, \binits{S.}}:
\batitle{Online learning and online convex optimization}.
\bjtitle{Foundations and Trends{\textregistered} in Machine Learning}
\bvolume{4}(\bissue{2}),
\bfpage{107}--\blpage{194}
(\byear{2012})
\doiurl{10.1561/2200000018}
\end{barticle}
\endbibitem

%%% 74
\bibitem[\protect\citeauthoryear{Schraudolph et~al.}{2007}]{Schraudolph2007}
\begin{bchapter}
\bauthor{\bsnm{Schraudolph}, \binits{N.N.}},
\bauthor{\bsnm{Yu}, \binits{J.}},
\bauthor{\bsnm{Günter}, \binits{S.}}:
\bctitle{A stochastic quasi-{N}ewton method for online convex optimization}.
In: \beditor{\bsnm{Meila}, \binits{M.}},
\beditor{\bsnm{Shen}, \binits{X.}} (eds.)
\bbtitle{Proceedings of the Eleventh International Conference on Artificial
  Intelligence and Statistics}.
\bsertitle{Proceedings of Machine Learning Research},
vol. \bseriesno{2},
pp. \bfpage{436}--\blpage{443}.
\bpublisher{PMLR},
\blocation{San Juan, Puerto Rico}
(\byear{2007})
\end{bchapter}
\endbibitem

%%% 75
\bibitem[\protect\citeauthoryear{Vose}{1991}]{Vose1991}
\begin{botherref}
\oauthor{\bsnm{Vose}, \binits{M.D.}}:
A linear algorithms for generating random numbers with a given distribution.
IEEE Transactions on Software Engineering
\textbf{17}(972)
(1991)
\doiurl{10.1109/32.92917}
\end{botherref}
\endbibitem

%%% 76
\bibitem[\protect\citeauthoryear{Wang and Banerjee}{2014}]{Wang2014}
\begin{barticle}
\bauthor{\bsnm{Wang}, \binits{H.}},
\bauthor{\bsnm{Banerjee}, \binits{A.}}:
\batitle{{Randomized block coordinate descent for online and stochastic
  optimization}}.
\bjtitle{arXiv preprint arXiv:1407.0107}
(\byear{2014})
\doiurl{10.48550/arXiv.1407.0107}
\end{barticle}
\endbibitem

%%% 77
\bibitem[\protect\citeauthoryear{Zinkevich}{2003}]{zinkevich2003online}
\begin{bchapter}
\bauthor{\bsnm{Zinkevich}, \binits{M.}}:
\bctitle{Online convex programming and generalized infinitesimal gradient
  ascent}.
In: \bbtitle{Proceedings of the Twentieth International Conference on
  International Conference on Machine Learning}.
\bsertitle{ICML'03},
pp. \bfpage{928}--\blpage{935}.
\bpublisher{AAAI Press},
\blocation{Washington, DC, USA}
(\byear{2003})
\end{bchapter}
\endbibitem

\end{thebibliography}

